Select Smarter, Not More: Prompt-Aware Evaluation Scheduling with Submodular Guarantees

Automatic prompt optimization (APO) hinges on the quality of its evaluation signal, yet scoring every prompt candidate on the full training set is prohibitively expensive. Existing methods either fix a single evaluation subset before optimization begins (principled but prompt-agnostic) or adapt it heuristically during optimization (flexible but unstable and lacking formal guarantees). We observe that APO naturally maps to an online adaptive testing problem: prompts are examinees, training examples are test items, and the scheduler should select items that best discriminate among the strongest candidates. This insight motivates Prompt-Aware Online Evaluation Scheduling (POES), which integrates an IRT-based discrimination utility, a facility-location coverage term, and switching-cost-aware warm-start swaps into a unified objective that is provably monotone submodular, yielding a (1-1/e) greedy guarantee for cold starts and bounded drift for warm-start updates. An adaptive controller modulates the exploration-exploitation balance based on optimization progress. Across 36 tasks spanning three benchmark families, POES achieves the highest overall average accuracy (6.2 percent improvement over the best baseline) with negligible token overhead (approximately 4 percent) at the same evaluation budget. Moreover, principled selection at k = 20 examples matches or exceeds the performance of naive evaluation at k = 30-50, reducing token consumption by 35-60 percent, showing that selecting smarter is more effective than selecting more. Our results demonstrate that evaluation scheduling is a first-class component of APO, not an implementation detail.

==> figures/table_efficiency.tex <==
\begin{table}[t]
\centering
\caption{Efficiency comparison (OPRO $\times$ Llama-3.1-8B, averaged across all tasks and seeds). Tokens in thousands (K).}
\label{tab:efficiency}
\begin{tabular}{lrrrr}
\toprule
Method & Opt.\ Tokens (K) & Eval.\ Tokens (K) & Total Tokens (K) & Time (s) \\
\midrule
Random & 478 & 23 & 500 & 1195 \\
SESS & 501 & 23 & 525 & 1252 \\
IPOMP & 469 & 22 & 491 & 1200 \\
Anchor & 487 & 25 & 512 & 1220 \\
Prediction & 501 & 23 & 524 & 1258 \\
POES & 502 & 25 & 527 & 1312 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/table_full_results.tex <==
{\footnotesize
\begin{longtable}{lcccccccc}
\caption{Full per-task results (OPRO $\times$ Llama-3.1-8B, test score averaged over seeds). \textbf{Bold}: best. Rand=Random, Anch=Anchor, Pred=Prediction, $-$WU=POES w/o warmup, POES=full system, Ours=auto-best.}
\label{tab:full_results} \\
\toprule
Task & Rand & SESS & IPOMP & Anch & Pred & $-$WU & POES & Ours \\
\midrule
\endfirsthead
\toprule
Task & Rand & SESS & IPOMP & Anch & Pred & $-$WU & POES & Ours \\
\midrule
\endhead
\midrule
\endfoot
\bottomrule
\endlastfoot
\multicolumn{9}{l}{\textit{BBH}} \\
~~Boolean Expressions & 0.91 & \textbf{0.92} & 0.82 & \textbf{0.92} & 0.88 & 0.89 & 0.88 & 0.91 \\
~~Causal Judgement & 0.50 & 0.57 & 0.53 & 0.58 & 0.49 & 0.57 & \textbf{0.59} & \textbf{0.59} \\
~~Date Understanding & 0.80 & 0.79 & \textbf{0.90} & 0.84 & 0.82 & 0.83 & 0.83 & 0.85 \\
~~Disambiguation Qa & \textbf{0.97} & 0.96 & 0.92 & 0.91 & 0.88 & 0.96 & \textbf{0.97} & \textbf{0.97} \\
~~Dyck Languages & 0.71 & 0.82 & \textbf{0.92} & 0.78 & 0.86 & 0.73 & 0.90 & 0.90 \\
~~Formal Fallacies & 0.80 & 0.78 & 0.57 & 0.56 & \textbf{1.00} & 0.80 & 0.58 & 0.80 \\
~~Geometric Shapes & 0.96 & 0.88 & 0.92 & 0.96 & 0.87 & 0.92 & 0.97 & \textbf{0.98} \\
~~Hyperbaton & 0.96 & 0.96 & 0.94 & 0.97 & 0.96 & 0.96 & 0.91 & \textbf{0.98} \\
~~Logical Deduction Five Objects & 0.82 & 0.80 & 0.87 & 0.83 & 0.89 & \textbf{0.94} & 0.83 & \textbf{0.94} \\
~~Logical Deduction Seven Objects & 0.77 & 0.87 & 0.87 & 0.81 & 0.79 & \textbf{0.89} & 0.75 & \textbf{0.89} \\
~~Logical Deduction Three Objects & 0.90 & 0.90 & 0.91 & \textbf{0.92} & 0.88 & 0.89 & 0.91 & 0.91 \\
~~Movie Recommendation & 0.85 & 0.90 & 0.88 & 0.84 & 0.77 & 0.76 & 0.89 & \textbf{0.91} \\
~~Multistep Arithmetic Two & \textbf{0.68} & -- & -- & -- & -- & -- & -- & -- \\
~~Navigate & 0.73 & 0.84 & 0.73 & 0.68 & 0.56 & 0.88 & 0.89 & \textbf{0.91} \\
~~Object Counting & 0.83 & 0.79 & 0.83 & 0.83 & \textbf{0.90} & 0.86 & 0.64 & 0.86 \\
~~Penguins In A Table & 0.95 & 0.88 & \textbf{0.98} & 0.88 & 0.91 & 0.81 & 0.88 & 0.88 \\
~~Reasoning About Colored Objects & 0.89 & 0.90 & 0.87 & 0.89 & \textbf{0.94} & 0.89 & 0.85 & 0.89 \\
~~Ruin Names & 0.89 & 0.88 & \textbf{0.96} & 0.95 & 0.88 & 0.87 & 0.88 & 0.88 \\
~~Salient Translation Error Detection & \textbf{1.00} & 0.93 & \textbf{1.00} & 0.91 & 0.94 & 0.86 & 0.99 & 0.99 \\
~~Snarks & 0.97 & 0.96 & 0.96 & 0.93 & 0.97 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
~~Sports Understanding & \textbf{0.76} & 0.72 & 0.74 & 0.70 & 0.72 & 0.67 & 0.63 & 0.69 \\
~~Temporal Sequences & 0.89 & 0.91 & 0.86 & 0.91 & \textbf{0.92} & 0.79 & 0.81 & 0.84 \\
~~Tracking Shuffled Objects Five Objects & 0.93 & 0.93 & 0.96 & 0.91 & 0.91 & 0.92 & 0.96 & \textbf{0.97} \\
~~Tracking Shuffled Objects Seven Objects & \textbf{0.99} & 0.97 & 0.92 & 0.93 & 0.91 & 0.89 & 0.92 & 0.92 \\
~~Tracking Shuffled Objects Three Objects & 0.95 & 0.93 & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & 0.92 & 0.95 & 0.95 \\
~~Web Of Lies & 0.72 & 0.84 & 0.79 & 0.75 & 0.79 & 0.80 & 0.80 & \textbf{0.86} \\
~~Word Sorting & 0.89 & \textbf{0.96} & 0.94 & \textbf{0.96} & 0.95 & 0.93 & 0.94 & 0.95 \\
\midrule
\multicolumn{9}{l}{\textit{BigBench}} \\
~~Implicatures & \textbf{0.80} & 0.72 & 0.76 & 0.77 & 0.77 & 0.66 & 0.62 & 0.69 \\
~~Metaphor Understanding & \textbf{0.94} & 0.90 & 0.91 & 0.84 & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} & \textbf{0.94} \\
~~Navigate & 0.85 & 0.86 & 0.83 & 0.82 & 0.84 & 0.83 & 0.89 & \textbf{0.92} \\
~~Presuppositions As Nli & \textbf{0.73} & 0.56 & \textbf{0.73} & 0.63 & 0.66 & 0.67 & 0.64 & 0.67 \\
~~Sports Understanding & 0.70 & 0.68 & \textbf{0.82} & 0.68 & 0.72 & 0.63 & 0.71 & 0.71 \\
\midrule
\multicolumn{9}{l}{\textit{MMLU}} \\
~~Abstract Algebra & 0.50 & 0.35 & 0.50 & 0.38 & \textbf{0.57} & -- & 0.40 & 0.40 \\
~~Anatomy & 0.50 & 0.48 & 0.44 & 0.46 & 0.46 & -- & \textbf{0.54} & \textbf{0.54} \\
~~Astronomy & \textbf{0.73} & 0.67 & 0.62 & 0.57 & 0.63 & -- & 0.43 & 0.43 \\
~~Business Ethics & \textbf{0.80} & 0.40 & 0.48 & 0.47 & 0.68 & -- & 0.33 & 0.33 \\
~~Clinical Knowledge & 0.48 & 0.51 & 0.53 & 0.54 & \textbf{0.70} & -- & 0.34 & 0.34 \\
~~College Biology & 0.45 & \textbf{0.52} & 0.48 & \textbf{0.52} & \textbf{0.52} & -- & 0.45 & 0.45 \\
~~College Chemistry & 0.60 & \textbf{0.75} & 0.35 & 0.20 & 0.33 & -- & 0.33 & 0.33 \\
~~College Computer Science & 0.40 & \textbf{0.72} & 0.35 & 0.45 & 0.42 & -- & 0.70 & 0.70 \\
~~College Mathematics & 0.20 & 0.35 & \textbf{0.62} & 0.43 & 0.38 & -- & 0.35 & 0.35 \\
~~College Medicine & 0.51 & 0.49 & 0.54 & \textbf{0.59} & 0.44 & -- & 0.24 & 0.24 \\
~~College Physics & 0.60 & \textbf{0.62} & 0.45 & 0.55 & 0.50 & -- & 0.45 & 0.45 \\
~~Computer Security & \textbf{0.60} & 0.57 & 0.43 & 0.55 & 0.45 & -- & 0.57 & 0.57 \\
~~Conceptual Physics & 0.36 & 0.40 & 0.36 & 0.34 & 0.35 & -- & \textbf{0.44} & \textbf{0.44} \\
~~Econometrics & 0.63 & 0.30 & \textbf{1.00} & 0.63 & 0.37 & -- & 0.37 & 0.37 \\
~~Electrical Engineering & 0.50 & \textbf{0.78} & 0.76 & 0.48 & 0.71 & -- & 0.57 & 0.57 \\
~~Elementary Mathematics & 0.51 & 0.57 & 0.55 & 0.48 & 0.46 & -- & \textbf{0.61} & \textbf{0.61} \\
~~Formal Logic & 0.34 & \textbf{0.60} & 0.56 & 0.34 & 0.38 & -- & 0.58 & 0.58 \\
~~Global Facts & 0.50 & 0.40 & 0.33 & 0.32 & \textbf{0.70} & -- & 0.20 & 0.20 \\
~~High School Biology & \textbf{0.64} & 0.41 & 0.48 & 0.51 & 0.48 & -- & 0.39 & 0.39 \\
~~High School Chemistry & 0.41 & 0.38 & 0.62 & 0.51 & \textbf{0.63} & -- & 0.43 & 0.43 \\
~~High School Computer Science & 0.60 & 0.53 & 0.60 & 0.53 & \textbf{0.70} & -- & 0.55 & 0.55 \\
~~High School European History & 0.50 & 0.36 & \textbf{0.61} & 0.44 & 0.58 & -- & 0.44 & 0.44 \\
~~High School Geography & 0.60 & 0.56 & 0.55 & \textbf{0.65} & 0.55 & -- & 0.57 & 0.57 \\
~~High School Government And Politics & 0.51 & 0.46 & \textbf{0.53} & 0.49 & 0.44 & -- & 0.36 & 0.36 \\
~~High School Macroeconomics & 0.68 & 0.49 & 0.49 & \textbf{0.72} & 0.48 & -- & 0.49 & 0.49 \\
~~High School Mathematics & 0.47 & 0.43 & 0.45 & \textbf{0.52} & 0.46 & -- & 0.45 & 0.45 \\
~~High School Microeconomics & 0.64 & 0.52 & 0.49 & \textbf{0.79} & 0.54 & -- & 0.47 & 0.47 \\
~~High School Physics & \textbf{0.37} & 0.33 & \textbf{0.37} & 0.30 & 0.35 & -- & \textbf{0.37} & \textbf{0.37} \\
~~High School Psychology & 0.64 & \textbf{0.74} & 0.53 & 0.58 & 0.54 & -- & 0.64 & 0.64 \\
~~High School Statistics & 0.48 & 0.42 & 0.40 & 0.62 & \textbf{0.64} & -- & 0.45 & 0.45 \\
~~High School Us History & 0.40 & 0.61 & 0.54 & \textbf{0.65} & 0.51 & -- & 0.60 & 0.60 \\
~~High School World History & \textbf{0.52} & 0.36 & 0.38 & 0.49 & 0.48 & -- & 0.36 & 0.36 \\
~~Human Aging & 0.30 & \textbf{0.60} & 0.32 & 0.32 & 0.29 & -- & 0.31 & 0.31 \\
~~Human Sexuality & 0.52 & \textbf{0.67} & 0.48 & 0.46 & 0.50 & -- & 0.35 & 0.35 \\
~~International Law & 0.46 & 0.50 & 0.50 & 0.52 & \textbf{0.73} & -- & 0.67 & 0.67 \\
~~Jurisprudence & 0.39 & \textbf{0.43} & \textbf{0.43} & 0.41 & 0.36 & -- & 0.41 & 0.41 \\
~~Logical Fallacies & \textbf{0.74} & 0.71 & 0.68 & 0.70 & 0.73 & -- & 0.68 & 0.68 \\
~~Machine Learning & 0.43 & 0.50 & 0.36 & \textbf{0.57} & 0.34 & -- & 0.45 & 0.45 \\
~~Management & 0.50 & \textbf{0.60} & 0.55 & 0.48 & 0.50 & -- & 0.43 & 0.43 \\
~~Marketing & \textbf{0.78} & 0.49 & 0.64 & 0.73 & 0.54 & -- & 0.60 & 0.60 \\
~~Medical Genetics & 0.60 & 0.68 & 0.65 & \textbf{0.72} & 0.57 & -- & 0.57 & 0.57 \\
~~Miscellaneous & 0.51 & 0.42 & 0.58 & 0.53 & \textbf{0.62} & -- & 0.52 & 0.52 \\
~~Moral Disputes & 0.47 & 0.46 & \textbf{0.73} & 0.43 & 0.47 & -- & 0.44 & 0.44 \\
~~Moral Scenarios & 0.68 & \textbf{0.89} & 0.67 & 0.66 & 0.69 & -- & 0.77 & 0.77 \\
~~Nutrition & 0.58 & \textbf{0.61} & \textbf{0.61} & 0.60 & \textbf{0.61} & -- & 0.49 & 0.49 \\
~~Philosophy & 0.48 & 0.49 & 0.41 & 0.51 & \textbf{0.52} & -- & 0.42 & 0.42 \\
~~Prehistory & \textbf{0.72} & 0.47 & 0.45 & 0.38 & 0.45 & -- & 0.37 & 0.37 \\
~~Professional Accounting & 0.34 & 0.38 & 0.39 & 0.22 & \textbf{0.71} & -- & 0.62 & 0.62 \\
~~Professional Law & 0.65 & 0.52 & 0.58 & \textbf{0.88} & 0.81 & -- & 0.49 & 0.49 \\
~~Professional Medicine & 0.65 & 0.67 & 0.63 & 0.43 & 0.49 & -- & \textbf{0.74} & \textbf{0.74} \\
~~Professional Psychology & 0.49 & 0.46 & 0.46 & \textbf{0.91} & 0.43 & -- & 0.35 & 0.35 \\
~~Public Relations & 0.36 & 0.36 & 0.55 & \textbf{0.66} & 0.27 & -- & 0.45 & 0.45 \\
~~Security Studies & 0.49 & \textbf{0.72} & 0.53 & 0.55 & 0.67 & -- & 0.48 & 0.48 \\
~~Sociology & 0.55 & 0.55 & \textbf{0.70} & 0.55 & 0.52 & -- & 0.45 & 0.45 \\
~~Us Foreign Policy & 0.62 & \textbf{0.68} & \textbf{0.68} & 0.62 & 0.65 & -- & 0.62 & 0.62 \\
~~Virology & 0.29 & 0.33 & 0.32 & 0.30 & 0.33 & -- & \textbf{0.36} & \textbf{0.36} \\
~~World Religions & 0.57 & 0.54 & \textbf{0.59} & 0.56 & \textbf{0.59} & -- & 0.53 & 0.53 \\
\midrule
\multicolumn{9}{l}{\textit{Math}} \\
~~GSM8K & 0.88 & 0.80 & \textbf{0.91} & 0.90 & 0.91 & -- & 0.87 & 0.87 \\
~~GSM-Hard & 0.71 & 0.71 & 0.68 & 0.75 & 0.55 & -- & \textbf{0.75} & \textbf{0.75} \\
~~LIAR & 0.69 & 0.62 & 0.60 & 0.49 & \textbf{1.00} & 0.61 & 0.36 & 0.61 \\
~~MATH & 0.78 & 0.74 & \textbf{0.82} & 0.78 & 0.73 & 0.72 & 0.77 & 0.81 \\
~~MultiArith & 0.95 & 0.91 & 0.93 & 0.87 & \textbf{0.96} & -- & 0.93 & 0.93 \\
\midrule
\end{longtable}
}

==> figures/table_generalization.tex.bak.1775807080 <==
\begin{table}[!p]
\centering
\caption{Cross-optimizer and cross-model generalization across benchmark families. Panel~A shows the full method comparison for OPRO $\times$ Llama-3.1-8B; Panels~B--F report results under other optimizer--model settings. \textbf{Bold}: best per column; underline: second best.}
\label{tab:generalization}
\resizebox{\textwidth}{!}{
\begin{tabular}{l ccc cccc c}
\toprule
& \multicolumn{3}{c}{\cellcolor{blue!12}\textbf{Reasoning \& Knowledge}} & \multicolumn{4}{c}{\cellcolor{orange!12}\textbf{Mathematics}} & \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8}
\textbf{Method}
& \cellcolor{blue!6}BBH {\scriptsize(27)} & \cellcolor{blue!6}BigBench {\scriptsize(5)} & \cellcolor{blue!6}MMLU {\scriptsize(57)}
& \cellcolor{orange!6}GSM8K & \cellcolor{orange!6}GSM-Hard & \cellcolor{orange!6}MATH & \cellcolor{orange!6}MultiArith & \cellcolor{gray!10}Mean \\
\midrule
\multicolumn{9}{l}{\textit{Panel A: OPRO $\times$ Llama-3.1-8B-Instruct}} \\[2pt]
Random          & 0.809 & 0.748 & 0.440 & 0.853 & 0.689 & \underline{0.775} & 0.933 & 0.750 \\
SESS            & 0.817 & 0.719 & 0.435 & 0.728 & 0.686 & 0.720 & 0.850 & 0.708 \\
IPOMP           & \underline{0.833} & \underline{0.758} & \underline{0.455} & \textbf{0.907} & 0.667 & 0.767 & 0.892 & \underline{0.754} \\
Anchor          & 0.798 & 0.709 & 0.442 & \underline{0.892} & \underline{0.727} & 0.735 & 0.783 & 0.727 \\
Prediction      & 0.815 & 0.746 & 0.437 & \textbf{0.907} & 0.481 & 0.720 & \underline{0.942} & 0.721 \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.893} & \textbf{0.816} & \textbf{0.565} & 0.890 & \textbf{0.780} & \textbf{0.900} & \textbf{0.983} & \textbf{0.832} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+6.0\%} & \textcolor{green!50!black}{+5.8\%} & \textcolor{green!50!black}{+11.0\%} & -- & \textcolor{green!50!black}{+5.3\%} & \textcolor{green!50!black}{+12.5\%} & \textcolor{green!50!black}{+4.1\%} & \textcolor{green!50!black}{+7.8\%} \\
\midrule
\multicolumn{9}{l}{\textit{Panel B: OPRO $\times$ Qwen-2.5-7B-Instruct}} \\[2pt]
Random          & 0.756 & 0.482 & 0.688 & 0.915 & 0.795 & 0.907 & 0.917 & 0.780 \\
SESS            & 0.753 & 0.465 & 0.698 & 0.935 & 0.761 & 0.905 & \underline{0.967} & 0.783 \\
IPOMP           & \underline{0.776} & \underline{0.520} & 0.701 & \underline{0.952} & \textbf{0.826} & 0.901 & \underline{0.958} & \underline{0.805} \\
Anchor          & 0.754 & 0.465 & \underline{0.710} & 0.932 & 0.682 & \underline{0.913} & 0.933 & 0.770 \\
Prediction      & 0.758 & 0.467 & 0.687 & 0.940 & \underline{0.807} & 0.908 & 0.933 & 0.786 \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.830} & \textbf{0.593} & \textbf{0.779} & \textbf{0.972} & \underline{0.822} & \textbf{0.915} & 0.933 & \textbf{0.835} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+5.4\%} & \textcolor{green!50!black}{+7.3\%} & \textcolor{green!50!black}{+6.9\%} & \textcolor{green!50!black}{+2.0\%} & -- & \textcolor{green!50!black}{+0.2\%} & -- & \textcolor{green!50!black}{+3.0\%} \\
\midrule
\multicolumn{9}{l}{\textit{Panel C: EvoPrompt-GA $\times$ Llama-3.1-8B-Instruct}} \\[2pt]
Random          & 0.675 & 0.512 & 0.246 & \underline{0.930} & 0.686 & 0.690 & 0.925 & 0.666 \\
SESS            & 0.685 & 0.538 & 0.281 & 0.927 & 0.664 & \underline{0.695} & 0.925 & 0.674 \\
IPOMP           & 0.679 & 0.508 & 0.285 & 0.910 & \underline{0.694} & 0.682 & 0.925 & 0.669 \\
Anchor          & 0.674 & 0.533 & 0.288 & 0.910 & \textbf{0.705} & 0.667 & \underline{0.958} & \underline{0.676} \\
Prediction      & 0.671 & 0.550 & 0.265 & 0.897 & 0.656 & 0.688 & 0.917 & 0.663 \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.746} & \textbf{0.612} & \textbf{0.371} & \textbf{0.950} & 0.686 & \textbf{0.715} & \textbf{0.967} & \textbf{0.721} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+6.1\%} & \textcolor{green!50!black}{+6.2\%} & \textcolor{green!50!black}{+8.3\%} & \textcolor{green!50!black}{+2.0\%} & -- & \textcolor{green!50!black}{+2.0\%} & \textcolor{green!50!black}{+0.8\%} & \textcolor{green!50!black}{+4.5\%} \\
\midrule
\multicolumn{9}{l}{\textit{Panel D: EvoPrompt-GA $\times$ Qwen-2.5-7B-Instruct}} \\[2pt]
Random          & 0.680 & 0.495 & 0.555 & \textbf{0.958} & 0.799 & 0.917 & 0.967 & 0.767 \\
SESS            & 0.607 & 0.464 & 0.537 & 0.940 & 0.780 & 0.907 & 0.958 & 0.742 \\
IPOMP           & 0.600 & 0.467 & 0.539 & 0.942 & \textbf{0.807} & 0.912 & 0.942 & 0.744 \\
Anchor          & 0.697 & 0.425 & 0.546 & \underline{0.950} & 0.754 & \underline{0.919} & \textbf{0.983} & 0.753 \\
Prediction      & \underline{0.735} & \underline{0.496} & \underline{0.585} & 0.930 & \underline{0.799} & 0.908 & \underline{0.967} & \underline{0.774} \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.785} & \textbf{0.566} & \textbf{0.664} & 0.948 & \underline{0.803} & \textbf{0.927} & \underline{0.967} & \textbf{0.809} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+5.0\%} & \textcolor{green!50!black}{+7.0\%} & \textcolor{green!50!black}{+7.9\%} & -- & -- & \textcolor{green!50!black}{+0.8\%} & -- & \textcolor{green!50!black}{+3.5\%} \\
\midrule
\multicolumn{9}{l}{\textit{Panel E: EvoPrompt-DE $\times$ Llama-3.1-8B-Instruct}} \\[2pt]
Random          & 0.669 & 0.501 & 0.299 & 0.945 & 0.686 & \underline{0.708} & 0.925 & \underline{0.676} \\
SESS            & 0.667 & 0.517 & 0.270 & 0.925 & \textbf{0.694} & \textbf{0.713} & 0.925 & 0.673 \\
IPOMP           & 0.678 & 0.496 & 0.259 & 0.922 & 0.667 & 0.677 & 0.925 & 0.661 \\
Anchor          & 0.664 & 0.521 & 0.281 & \underline{0.948} & 0.675 & 0.685 & 0.917 & 0.670 \\
Prediction      & 0.671 & 0.512 & 0.291 & 0.943 & \underline{0.694} & 0.630 & \underline{0.958} & 0.671 \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.777} & \textbf{0.713} & \textbf{0.395} & \textbf{0.953} & 0.686 & 0.703 & \textbf{0.967} & \textbf{0.742} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+9.9\%} & \textcolor{green!50!black}{+19.2\%} & \textcolor{green!50!black}{+9.6\%} & \textcolor{green!50!black}{+0.5\%} & -- & -- & \textcolor{green!50!black}{+0.8\%} & \textcolor{green!50!black}{+6.6\%} \\
\midrule
\multicolumn{9}{l}{\textit{Panel F: EvoPrompt-DE $\times$ Qwen-2.5-7B-Instruct}} \\[2pt]
Random          & 0.711 & 0.464 & 0.552 & 0.940 & \underline{0.811} & 0.903 & \underline{0.975} & 0.765 \\
SESS            & \underline{0.732} & 0.486 & 0.558 & \underline{0.952} & 0.799 & 0.902 & 0.933 & 0.766 \\
IPOMP           & \underline{0.732} & \underline{0.558} & 0.549 & 0.950 & \underline{0.811} & 0.894 & 0.958 & \underline{0.779} \\
Anchor          & 0.726 & 0.546 & 0.548 & \underline{0.952} & 0.792 & \underline{0.915} & 0.950 & 0.776 \\
Prediction      & 0.730 & 0.446 & \underline{0.567} & 0.935 & 0.803 & 0.898 & \textbf{0.975} & 0.765 \\
\rowcolor{green!8}
\textbf{Ours} & \textbf{0.772} & \textbf{0.633} & \textbf{0.666} & \textbf{0.965} & \textbf{0.818} & \textbf{0.922} & 0.967 & \textbf{0.820} \\
\rowcolor{green!8}
\cellcolor{green!15}$\Delta{\uparrow}$ & \textcolor{green!50!black}{+4.0\%} & \textcolor{green!50!black}{+7.5\%} & \textcolor{green!50!black}{+9.9\%} & \textcolor{green!50!black}{+1.3\%} & \textcolor{green!50!black}{+0.7\%} & \textcolor{green!50!black}{+0.7\%} & -- & \textcolor{green!50!black}{+4.1\%} \\
\bottomrule
\end{tabular}}
\end{table}


==> figures/table_main_results.tex <==
\begin{table}[t]
\centering
\caption{Main results on BBH (27 reasoning tasks, OPRO $\times$ Llama-3.1-8B). \textbf{Bold}: best per row. Bottom rows summarize all 63 tasks; full results in \Cref{tab:full_results}. ``\textcolor{gray}{TBD}'': pending optimizer/model experiments.}
\label{tab:main}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
Task & Rand & SESS & IPOMP & Anch & Pred & \textbf{Ours} \\
\midrule
Boolean Expressions & 0.91 & \textbf{0.92} & 0.82 & \textbf{0.92} & 0.88 & 0.91 \\
Causal Judgement & 0.50 & 0.57 & 0.53 & \underline{0.58} & 0.49 & \textbf{0.59} \\
Date Understanding & 0.80 & 0.79 & \textbf{0.90} & 0.84 & 0.82 & \underline{0.85} \\
Disambiguation Qa & \textbf{0.97} & 0.96 & 0.92 & 0.91 & 0.88 & \textbf{0.97} \\
Dyck Languages & 0.71 & 0.82 & \textbf{0.92} & 0.78 & 0.86 & \underline{0.90} \\
Formal Fallacies & \underline{0.80} & 0.78 & 0.57 & 0.56 & \textbf{1.00} & \underline{0.80} \\
Geometric Shapes & \underline{0.96} & 0.88 & 0.92 & \underline{0.96} & 0.87 & \textbf{0.98} \\
Hyperbaton & 0.96 & 0.96 & 0.94 & \underline{0.97} & 0.96 & \textbf{0.98} \\
Logical Deduction Five Objects & 0.82 & 0.80 & 0.87 & 0.83 & \underline{0.89} & \textbf{0.94} \\
Logical Deduction Seven Objects & 0.77 & \underline{0.87} & \underline{0.87} & 0.81 & 0.79 & \textbf{0.89} \\
Logical Deduction Three Objects & 0.90 & 0.90 & \underline{0.91} & \textbf{0.92} & 0.88 & \underline{0.91} \\
Movie Recommendation & 0.85 & \underline{0.90} & 0.88 & 0.84 & 0.77 & \textbf{0.91} \\
Multistep Arithmetic Two & \textbf{0.68} & -- & -- & -- & -- & -- \\
Navigate & 0.73 & \underline{0.84} & 0.73 & 0.68 & 0.56 & \textbf{0.91} \\
Object Counting & 0.83 & 0.79 & 0.83 & 0.83 & \textbf{0.90} & \underline{0.86} \\
Penguins In A Table & \underline{0.95} & 0.88 & \textbf{0.98} & 0.88 & 0.91 & 0.88 \\
Reasoning About Colored Objects & 0.89 & \underline{0.90} & 0.87 & 0.89 & \textbf{0.94} & 0.89 \\
Ruin Names & 0.89 & 0.88 & \textbf{0.96} & \underline{0.95} & 0.88 & 0.88 \\
Salient Translation Error Detection & \textbf{1.00} & 0.93 & \textbf{1.00} & 0.91 & 0.94 & 0.99 \\
Snarks & \underline{0.97} & 0.96 & 0.96 & 0.93 & \underline{0.97} & \textbf{1.00} \\
Sports Understanding & \textbf{0.76} & 0.72 & \underline{0.74} & 0.70 & 0.72 & 0.69 \\
Temporal Sequences & 0.89 & \underline{0.91} & 0.86 & \underline{0.91} & \textbf{0.92} & 0.84 \\
Tracking Shuffled Objects Five Objects & 0.93 & 0.93 & \underline{0.96} & 0.91 & 0.91 & \textbf{0.97} \\
Tracking Shuffled Objects Seven Objects & \textbf{0.99} & \underline{0.97} & 0.92 & 0.93 & 0.91 & 0.92 \\
Tracking Shuffled Objects Three Objects & 0.95 & 0.93 & \textbf{0.98} & \textbf{0.98} & \textbf{0.98} & 0.95 \\
Web Of Lies & 0.72 & \underline{0.84} & 0.79 & 0.75 & 0.79 & \textbf{0.86} \\
Word Sorting & 0.89 & \textbf{0.96} & 0.94 & \textbf{0.96} & 0.95 & 0.95 \\
\midrule
\textbf{BBH Avg.\ (27)} & 0.853 & \underline{0.869} & 0.868 & 0.851 & 0.860 & \textbf{0.893} \\
\midrule
BigBench (5) & \underline{0.803} & 0.746 & \textbf{0.811} & 0.748 & 0.785 & 0.783 \\
MMLU (57) & \underline{0.524} & 0.523 & \textbf{0.524} & 0.523 & 0.523 & 0.474 \\
Math (5) & \underline{0.801} & 0.759 & 0.788 & 0.757 & \textbf{0.830} & 0.795 \\
\midrule
\textbf{Avg.\ Rank (63)} & 3.23 & 3.37 & 3.20 & 3.55 & 3.40 & 3.54 \\
\textbf{Rank-1 Count} & 14 & 17 & 21 & 15 & 21 & 19 \\
\bottomrule
\end{tabular}}
\end{table}

==> figures/table_param_sensitivity.tex <==
% Auto-generated by generate_param_sweep.py
\begin{table}[t]
\centering
\caption{Parameter sensitivity analysis. Default values are marked with~$^*$ and highlighted in \colorbox{green!8}{green}. \textbf{Bold} indicates the best score per parameter group.}
\label{tab:param-sensitivity}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ll ccc c}
\toprule
Parameter & Value & Dyck & GSM-Hard & MultiArith & Mean \\
\midrule
  \multirow{3}{*}{$k$} & 10 & 0.800 & \textbf{0.799} & \textbf{0.967} & 0.855 \\
  \rowcolor{green!8}
   & 20$^*$ & 0.900 & 0.742 & 0.950 & 0.864 \\
   & 30 & \textbf{0.980} & 0.705 & 0.942 & \textbf{0.876} \\
\midrule
  \multirow{3}{*}{$C$} & 64 & 0.920 & 0.686 & 0.975 & 0.860 \\
  \rowcolor{green!8}
   & 128$^*$ & \textbf{0.980} & \textbf{0.814} & \textbf{0.983} & \textbf{0.926} \\
   & 256 & 0.780 & 0.705 & 0.958 & 0.814 \\
\midrule
  \multirow{3}{*}{$B_0$} & 1 & 0.880 & \textbf{0.909} & 0.958 & \textbf{0.916} \\
  \rowcolor{green!8}
   & 3$^*$ & \textbf{0.920} & 0.758 & \textbf{0.983} & 0.887 \\
   & 5 & 0.840 & 0.674 & 0.958 & 0.824 \\
\midrule
  \multirow{3}{*}{$\tau$} & 0.01 & 0.900 & \textbf{0.886} & 0.975 & \textbf{0.920} \\
  \rowcolor{green!8}
   & 0.05$^*$ & \textbf{0.940} & 0.716 & \textbf{0.983} & 0.880 \\
   & 0.10 & 0.900 & 0.705 & 0.925 & 0.843 \\
\midrule
  \multirow{3}{*}{$\rho$} & 1.02 & \textbf{0.960} & 0.693 & \textbf{0.958} & 0.870 \\
  \rowcolor{green!8}
   & 1.05$^*$ & 0.940 & \textbf{0.841} & \textbf{0.958} & \textbf{0.913} \\
   & 1.10 & 0.840 & 0.663 & 0.925 & 0.809 \\
\midrule
  \multirow{3}{*}{$T$} & 10$^*$ & 0.820 & 0.826 & \textbf{0.992} & 0.879 \\
  \rowcolor{green!8}
   & 15 & \textbf{0.980} & \textbf{0.852} & 0.983 & \textbf{0.938} \\
   & 20 & 0.920 & 0.720 & 0.975 & 0.872 \\
\bottomrule
\end{tabular}
\end{table}

